RLBoost: Boosting Supervised Models using Deep Reinforcement Learning

Data quality or data evaluation is sometimes a task as important as collecting a large volume of data when it comes to generating accurate artificial intelligence models. In fact, being able to evaluate the data can lead to a larger database that is better suited to a particular problem because we have the ability to filter out data obtained automatically of dubious quality. In this paper we present RLBoost, an algorithm that uses deep reinforcement learning strategies to evaluate a particular dataset and obtain a model capable of estimating the quality of any new data in order to improve the final predictive quality of a supervised learning model. This solution has the advantage that of being agnostic regarding the supervised model used and, through multi-attention strategies, takes into account the data in its context and not only individually. The results of the article show that this model obtains better and more stable results than other state-of-the-art algorithms such as LOO, DataShapley or DVRL.

==> tables/legacy/4.1.aucs_table.tex <==


\begin{table}[H]
    \caption{Table of AUCs detecting noisy data by each of the models in the tabular data sets}
    \begin{adjustwidth}{-4cm}{-4cm}
    \footnotesize
    \centering
    \begin{tabular}{@{}ll||ccc|cccc@{}}
    \toprule
    \textbf{Data}                  & \textbf{Noise \%}  & \textbf{LOO}        & \textbf{SHAP}       & \textbf{DVRL}        & \textbf{\begin{tabular}[c]{@{}l@{}}RLB\\ (c2=1e-1)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}RLB\\ (c2=1e-2)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}RLB\\ (c2=1e-3)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}RLB\\ (c2=1e-4)\end{tabular}} \\ \midrule
    \multirow{3}{*}{\textit{Adult}}   & 15              & $0.339 (\pm 0.0)$   & $0.729 (\pm 0.018)$ & $0.657 (\pm 0.193)$  & $0.816 (\pm 0.006)$                                                 & $\mathbf{0.831 (\pm 0.01)}$                                         &  $0.815 (\pm 0.009)$                                                &  $0.828 (\pm 0.008)$                                                \\  
                                      & 30              & $0.509 (\pm 0.0)$   & $0.724 (\pm 0.019)$ & $0.734 (\pm 0.195)$  & $\mathbf{0.856 (\pm 0.009)}$                                        & $0.825 (\pm 0.015)$                                                 &  $0.839 (\pm 0.008)$                                                &  $0.819 (\pm 0.013)$                                                \\ \midrule

    \multirow{3}{*}{\textit{A5A}}     & 15              & $0.688 (\pm 0.0)$   & -----               & $0.791 (\pm 0.141)$  & $0.833 (\pm 0.016)$                                                 & $\mathbf{0.845 (\pm 0.007)}$                                        &  $0.833 (\pm 0.008)$                                                &  $0.819 (\pm 0.007)$                                                \\  
                                      & 30              & $0.535 (\pm 0.0)$   & -----               & $0.68 (\pm 0.167)$   & $0.847 (\pm 0.007)$                                                 & $\mathbf{0.86 (\pm 0.005)}$                                         &  $0.845 (\pm 0.006)$                                                &  $0.832 (\pm 0.018)$                                                \\ \midrule

    \multirow{3}{*}{\textit{W5A}}     & 15              & $0.628 (\pm 0.0)$   & -----               & $0.946 (\pm 0.008)$  & $\mathbf{0.957 (\pm 0.013)}$                                        & $0.947 (\pm 0.008)$                                                 &  $0.916 (\pm 0.008)$                                                &  $0.887 (\pm 0.007)$                                                \\  
                                      & 30              & $0.455 (\pm 0.0)$   & -----               & $0.859 (\pm 0.185)$  & $\mathbf{0.967 (\pm 0.003)}$                                        & $0.967 (\pm 0.006)$                                                 &  $0.933 (\pm 0.006)$                                                &  $0.892 (\pm 0.025)$                                                \\ \midrule

    \multirow{3}{*}{\textit{CIFAR10}} & 15              & $0.619 (\pm 0.0)$   & -----               & $0.548 (\pm 0.061)$  & $0.757 (\pm 0.014)$                                                 & $\mathbf{0.779 (\pm 0.044)}$                                        &  $0.764 (\pm 0.019)$                                                &  $0.657 (\pm 0.021)$                                                \\  
                                      & 30              & $0.592 (\pm 0.0)$   & -----               & $0.498 (\pm 0.003)$  & $0.767 (\pm 0.005)$                                                 & $\mathbf{0.855 (\pm 0.005)}$                                        &  $0.82 (\pm 0.009)$                                                 &  $0.678 (\pm 0.021)$                                                \\ \bottomrule
    
    \end{tabular}
    \end{adjustwidth}
    \label{table:tab_aucs}
\end{table}


==> tables/legacy/4.1.score_table.tex <==


\begin{table}[H]
    \caption{Table of scores against test data using the final filtering proposed by each of the models in the tabular data sets}
    \begin{adjustwidth}{-4cm}{-4cm}
    \footnotesize
    \centering
    \begin{tabular}{@{}ll||cccc|cccc@{}}
    \toprule
    \textbf{Data}                  & \textbf{Noise \%} & \textbf{Baseline}   & \textbf{LOO}      & \textbf{SHAP}      & \textbf{DVRL}                   & \textbf{\begin{tabular}[c]{@{}l@{}}RLB\\ (c2=1e-1)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}RLB\\ (c2=1e-2)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}RLB\\ (c2=1e-3)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}RLB\\ (c2=1e-4)\end{tabular}} \\ \midrule
    \multirow{3}{*}{\textit{Adult}}   & 0              & $\mathbf{0.832}$    & $0.832(\pm0.0)$   & $0.832(\pm0.0)$    &  $0.832(\pm0.000)$              & $0.807(\pm0.006)$                                                   & $0.814(\pm0.005)$                                                   & $0.813(\pm0.001)$                                                   &  $0.814(\pm0.002)$                                                  \\  
                                      & 15             & $\mathbf{0.814}$    & $0.814(\pm0.0)$   & $0.814(\pm0.0)$    &  $0.793(\pm0.029)$              & $0.799(\pm0.008)$                                                   & $0.811(\pm0.006)$                                                   & $0.816(\pm0.004)$                                                   &  $0.812(\pm0.005)$                                                  \\  
                                      & 30             & $0.776$             & $0.776(\pm0.0)$   & $0.776(\pm0.0)$    &  $0.768(\pm0.007)$              & $0.813(\pm0.004)$                                                   & $0.812(\pm0.007)$                                                   & $\mathbf{0.814(\pm0.001)}$                                          &  $0.814(\pm0.007)$                                                  \\ \midrule

    \multirow{3}{*}{\textit{A5A}}     & 0              & $\mathbf{0.844}$    & $0.844(\pm0.0)$   & -----              &  $0.828(\pm0.002)$              & $0.834(\pm0.004)$                                                   & $0.833(\pm0.002)$                                                   & $0.827(\pm0.003)$                                                   &  $0.826(\pm0.002)$                                                  \\  
                                      & 15             & $\mathbf{0.838}$    & $0.838(\pm0.0)$   & -----              &  $0.829(\pm0.004)$              & $0.831(\pm0.004)$                                                   & $0.830(\pm0.004)$                                                   & $0.826(\pm0.002)$                                                   &  $0.825(\pm0.004)$                                                  \\  
                                      & 30             & $0.807$             & $0.807(\pm0.0)$   & -----              &  $0.809(\pm0.016)$              & $0.826(\pm0.006)$                                                   & $\mathbf{0.831(\pm0.003)}$                                          & $0.823(\pm0.006)$                                                   &  $0.826(\pm0.001)$                                                  \\ \midrule

    \multirow{3}{*}{\textit{W5A}}     & 0              & $\mathbf{0.982}$    & $0.982(\pm0.0)$   & -----              &  $0.979(\pm0.004)$              & $0.979(\pm0.001)$                                                   & $0.974(\pm0.006)$                                                   & $0.980(\pm0.001)$                                                   &  $0.981(\pm0.001)$                                                  \\  
                                      & 15             & $\mathbf{0.977}$    & $0.977(\pm0.0)$   & -----              &  $0.970(\pm0.004)$              & $0.970(\pm0.007)$                                                   & $0.972(\pm0.005)$                                                   & $0.969(\pm0.004)$                                                   &  $0.970(\pm0.005)$                                                  \\  
                                      & 30             & $0.946$             & $0.946(\pm0.0)$   & -----              &  $0.899(\pm0.096)$              & $0.959(\pm0.005)$                                                   & $\mathbf{0.966(\pm0.005)}$                                          & $0.961(\pm0.002)$                                                   &  $0.957(\pm0.005)$                                                  \\ \midrule

    \multirow{3}{*}{\textit{CIFAR10}} & 0              & $0.880$             & $0.890(\pm0.0)$   & -----              &  $0.866(\pm0.031)$              & $0.896(\pm0.003)$                                                   & $0.902(\pm0.006)$                                                   & $\mathbf{0.902(\pm0.002)}$                                          &  $0.898(\pm0.004)$                                                  \\  
                                      & 15             & $0.781$             & $0.759(\pm0.0)$   & -----              &  $0.748(\pm0.017)$              & $0.855(\pm0.007)$                                                   & $0.869(\pm0.016)$                                                   & $\mathbf{0.882(\pm0.014)}$                                          &  $0.873(\pm0.014)$                                                  \\  
                                      & 30             & $0.683$             & $0.648(\pm0.0)$   & -----              &  $0.648(\pm0.010)$              & $0.797(\pm0.007)$                                                   & $0.860(\pm0.007)$                                                   & $\mathbf{0.879(\pm0.011)}$                                          &  $0.866(\pm0.007)$                                                  \\ \bottomrule
    
    \end{tabular}
    \end{adjustwidth}
    \label{table:tab_scores}
\end{table}


==> tables/legacy/4.2.aucs_table.tex <==


\begin{table}[H]
    \caption{Table of AUCs detecting noisy data by each of the models in image dataset}
    \begin{adjustwidth}{-4cm}{-4cm}
    \footnotesize
    \centering
    \begin{tabular}{@{}ll||ccc|cccc@{}}
    \toprule
    \textbf{Data}                  & \textbf{Noise \%}  & \textbf{LOO}        & \textbf{SHAP}       & \textbf{DVRL}                 & \textbf{\begin{tabular}[c]{@{}l@{}}RLB\\ (c2=1e-1)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}RLB\\ (c2=1e-2)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}RLB\\ (c2=1e-3)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}RLB\\ (c2=1e-4)\end{tabular}} \\ \midrule
    \multirow{3}{*}{\textit{MNIST}}   & 15              & $0.440(\pm0.0)$     & -                   & $0.884(\pm0.192)$             & $0.816 (\pm 0.006)$                                                 & $\mathbf{0.853(\pm0.014)}$                                          & $0.839(\pm0.014)$                                                   & $0.679(\pm0.013)$                                                   \\  
                                      & 30              & $0.575(\pm0.0)$     & -                   & $\mathbf{0.977(\pm0.006)}$    & $0.737(\pm0.03)$                                                    & $0.861(\pm0.012)$                                                   & $0.843(\pm0.012)$                                                   & $0.688(\pm0.016)$                                                   \\ \bottomrule
    
    \end{tabular}
    \end{adjustwidth}
    \label{table:tab_aucs_mnist}
\end{table}

==> tables/legacy/4.2.score_table.tex <==


\begin{table}[H]
    \caption{Table of scores against test data using the final filtering proposed by each of the models in the MNIST data set}
    \begin{adjustwidth}{-4cm}{-4cm}
    \footnotesize
    \centering
    \begin{tabular}{@{}ll||cccc|cccc@{}}
    \toprule
    \textbf{Data}                  & \textbf{Noise \%} & \textbf{Baseline} & \textbf{LOO}       & \textbf{SHAP} & \textbf{DVRL}       & \textbf{\begin{tabular}[c]{@{}l@{}}RLB\\ (c2=1e-1)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}RLB\\ (c2=1e-2)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}RLB\\ (c2=1e-3)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}RLB\\ (c2=1e-4)\end{tabular}} \\ \midrule
    \multirow{3}{*}{\textit{MNIST}}& $0$               & $\mathbf{0.968}$  & $0.968(\pm0.000)$  & -             & $0.908(\pm0.119)$   & $0.967(\pm0.001)$                                                        & $0.968(\pm0.002)$                                              & $0.969(\pm0.002)$                                                   & $0.968(\pm0.001)$                                                   \\ 
                                   & $15$              & $0.779$           & $0.780(\pm0.000)$  & -             & $0.923(\pm0.081)$   & $0.890(\pm0.013)$                                                        & $0.910(\pm0.007)$                                              & $\mathbf{0.914(\pm0.009)}$                                          & $0.876(\pm0.011)$                                                   \\  
                                   & $30$              & $0.621$           & $0.620(\pm0.000)$  & -             & $0.780(\pm0.379)$   & $0.782(\pm0.017)$                                                        & $0.842(\pm0.016)$                                              & $\mathbf{0.867(\pm0.018)}$                                                   & $0.802(\pm0.030)$                                                   \\ \midrule
    \end{tabular}
    \end{adjustwidth}
    \label{table:img_scores}
\end{table}
    
